TOPCAT: Desktop Exploration of Tabular Data for Astronomy and Beyond

TOPCAT, the Tool for OPerations on Catalogues And Tables, is an interactive desktop application for retrieval, analysis and manipulation of tabular data, offering a powerful and flexible range of interactive visualization options amongst other features. Its visualization capabilities focus on enabling interactive exploration of large static local tables - millions of rows and hundreds of columns can easily be handled on a standard desktop or laptop machine, and various options are provided for meaningful graphical representation of such large datasets. TOPCAT has been developed in the context of astronomy, but many of its features are equally applicable to other domains. The software, which is free and open source, is written in Java, and the underlying high-performance visualisation library is suitable for re-use in other applications.

==> makefile <==
.SUFFIXES: .tex .eps .ps .pdf .png .view

PAPER = topcatviz
STILTS_JAR = stilts.jar
STILTS = java -jar $(STILTS_JAR)
TEXLIVE = /mbt/local/texlive/2015/bin/x86_64-linux
LATEX = $(TEXLIVE)/pdflatex
BIBTEX = $(TEXLIVE)/bibtex
BUILT_FIGURES = fig-link-a.pdf fig-link-b.pdf fig-multid.pdf \
                fig-vectors2.pdf \
                fig-cloud.png fig-weight.png fig-histo.pdf
CLOUD_PANELS = cmd-flat.png cmd-tran.png cmd-cont.png \
               cmd-grid.png cmd-dens.png cmd-auto.png
WEIGHT_PANELS = cmd-waux.png cmd-wgri.png cmd-weig.png
CMD_DATA = bellini.fits cloud-point.csv weight-point.csv
ARCHIVE_FILES = $(PAPER).tex $(PAPER).bib $(PAPER).bbl $(PAPER).pdf \
                changes.txt \
                fig-multid.pdf fig-vectors2.pdf fig-link-a.pdf fig-link-b.pdf \
                fig-activation2.png fig-cloud.png fig-weight.png \
                fig-histo.pdf plotwin_pos.png plotwin_control.png \
                mw.pdf fig-pognonec-drymass.png fig-rydberg.pdf \
                mdpi.cls logo-mdpi.pdf logo-ccby.pdf

build: $(PAPER).pdf

view: $(PAPER).view

clean:
	rm -f $(PAPER).{aux,bbl,blg,log,out,pdf,zip}
	rm -f $(BUILT_FIGURES) $(CLOUD_PANELS) $(WEIGHT_PANELS)
	rm -f cloud-point.csv weight-point.csv

.eps.pdf:
	ps2pdf $<

.pdf.view:
	test -f $< && acroread -geometry +50+50 -openInNewWindow $<

.png.view:
	test -f $< && xv $<


$(PAPER).pdf: $(PAPER).tex $(PAPER).bib \
              logo-mdpi.pdf logo-ccby.pdf informatics-logo.pdf \
              $(BUILT_FIGURES)
	$(LATEX) $(PAPER) \
        && $(BIBTEX) $(PAPER) \
        && $(LATEX) $(PAPER) \
        && $(LATEX) $(PAPER) \
        || rm -f $@ $(PAPER).bbl $(PAPER).blg

#$(PAPER).pdf: $(PAPER).tex \
#              logo-mdpi.pdf logo-ccby.pdf informatics-logo.pdf \
#              $(BUILT_FIGURES)
#	$(LATEX) $(PAPER) \
#        && $(LATEX) $(PAPER) \
#        && $(LATEX) $(PAPER) \
#        || rm -f $@

archive: $(PAPER).zip

$(PAPER).zip: $(ARCHIVE_FILES)
	jar cfM $@ $(ARCHIVE_FILES)

$(STILTS_JAR): 
	curl ftp://andromeda.star.bris.ac.uk/pub/star/stilts/v3.1/stilts.jar \
             >$@

hsoy_pleiades_nocluster.fits: $(STILTS_JAR)
	$(STILTS) tapquery \
                  sync=true \
                  tapurl='http://dc.g-vo.org/tap' \
                  adql="select raj2000, dej2000, \
                        pmra, pmde, jmag, hmag, kmag \
                        from hsoy.main \
                        where 1=CONTAINS(POINT('',56.75, 24.117), \
                                         CIRCLE('', raj2000, dej2000, 3))" \
                   maxrec=200000 \
                   out=$@

fig-link-a.pdf: hsoy_pleiades.fits $(STILTS_JAR)
	$(STILTS) plot2plane \
               xpix=400 ypix=400 \
               in=hsoy_pleiades.fits x='pmra*36e5' y='pmde*36e5' \
               icmd2='select cluster' \
               layer1=mark shading1=density denseclip1=0,0.5 color1=lightgrey \
               layer2=mark shading2=flat color2=red shape2=open_circle size2=2 \
               layer3=contour nlevel=5 scaling=log smooth=10 color=grey \
               leglabel1=All leglabel2=Cluster \
               xmin=-42 xmax=55 ymin=-65 ymax=35 \
               xlabel='{\Large\mu_\alpha*}\,/\,{\sf mas.yr^{-1}}' \
               ylabel='{\Large\mu_\delta}\,/\,{\sf mas.yr^{-1}}' \
               texttype=latex fontsize=16 legpos='0.95,0.95' minor=false \
               seq=1,2 \
               out=$@

fig-link-b.pdf: hsoy_pleiades.fits $(STILTS_JAR)
	$(STILTS) plot2plane \
               xpix=400 ypix=400 \
               in=hsoy_pleiades.fits x=jmag-kmag y=kmag \
               icmd2='select cluster' \
               layer1=mark shading1=density denseclip1=0,0.5 color1=lightgrey \
               layer2=mark shading2=flat color2=red shape2=open_circle size2=2 \
               leglabel1=All leglabel2=Cluster \
               xmin=-0.41 xmax=1.95 ymin=3.8 ymax=17 \
               texttype=latex fontsize=16 legpos='0.95,0.95' minor=false \
               yflip=true \
               out=$@ 

fig-igsl.pdf: $(STILTS_JAR)
	$(STILTS) -bench plot2sky \
               xpix=2000 ypix=1000 fontsize=36 \
               crowd=1 projection=aitoff datasys=equatorial viewsys=galactic \
               layer1=skydensity lon1=raj2000 lat1=dej2000 \
               combine1=count level1=7 in1=/mbt/bigdata/igsl/igsl3.colfits \
               auxfunc=log auxmap=viridis \
               icmd1=progress storage=simple \
               out=$@

EVANTHIA_CMD = $(STILTS) plot2plane \
             in=evanthia_Table1.vot \
             xpix=500 ypix=400 \
             x=starburst_indicator xlog=true \
             y=AGN_indicator yflip=true \
             size='min(AGN_Contribution,20)' \
             autoscale=true scale=0.5 \
             shading=aux aux=Luminosity/1e32 auxfunc=log \
             auxmap=cubehelix auxflip=false auxclip=0,.9 \
             layer.o=size icmd.o='select obscured' shape.o=open_circle \
             layer.u=size icmd.u='select unobscured' shape.u=filled_circle \
             layer.l=function axis.l=vertical fexpr.l=0.2 color.l=black \
                              thick.l=2 dash.l=dash antialias.l=true \
             legpos=.1,.9 leglabel.o=Obscured leglabel.u=Unobscured \
                          legseq=.o,.u \
             seq=.u,.o,.l \
             texttype=latex fontsize=20 \
             xlabel="EW_{11.2\mu m}" ylabel="S_{sil} [IRS]" \
             auxlabel="L_{7\mu m}[L_{\odot}]" \

evanthia: $(STILTS_JAR)
	$(EVANTHIA_CMD)

fig-evanthia.pdf: $(STILTS_JAR)
	$(EVANTHIA_CMD) out=$@

gavo_g2.fits:
	cp /mbt/data/plot2data/gavo_g2.fits $@

fig-vectors2.pdf: $(STILTS_JAR) gavo_g2.fits
	$(STILTS) plot2cube \
        legend=false zoom=1.2 \
        xmin=6.2 xmax=7.7 ymin=12.7 ymax=13.8 zmin=23.6 zmax=25.2 \
        xcrowd=1.5 ycrowd=1.5 zcrowd=1.5 \
        xlabel= xpix=400 ypix=400 auxvisible=false \
        in=gavo_g2.fits \
        x=x y=y z=z shading=aux aux=redshift \
        opaque=2 auxmap=red-blue \
        layer1=xyzvector xdelta1=velx ydelta1=vely zdelta1=velz scale1=1.4 \
        layer2=mark size2=1 shape2=open_circle \
        seq=1 auxflip=true auxfunc=sqrt \
        out=$@

fig-multid.pdf: $(STILTS_JAR)
	$(STILTS) plot2plane \
                  in1=/mbt/data/survey/dr5qso.fits \
                  layer1=sizexy shape1=filled_ellipse \
                  x1=psfmag_u-psfmag_g y1=psfmag_r-psfmag_z \
                  xsize1='exp(psfmag_g)' ysize1='exp(psfmag_r)' \
                  xmin=-3 xmax=1 ymin=1 ymax=3.2 \
                  shading1=aux aux1=6-z auxfunc=log \
                  auxmax=3 scale1=1.3 auxmap=cubehelix \
                  xlabel=umag-gmag ylabel=rmag-zmag auxlabel='' \
                  out=$@

fig-histo.pdf: $(STILTS_JAR)
	$(STILTS) plot2plane \
               in=/mbt/data/survey/tgas_source.fits \
               x='hypot(pmra_error,pmdec_error)' \
               xlog=true normalise=maximum \
               layer1=histogram color1=red \
               layer2=kde color2=blue \
               layer3=densogram densemap3=heat densefunc3=log denseclip=0,1 \
               size3=50 pos3=.5 \
               ylabel='{\sf Normalised\ frequency}' xlabel='|\mu|' \
               texttype=latex fontsize=16 minor=false \
               xpix=700 ypix=300 \
               out=$@

bellini.fits: $(STILTS_JAR)
	$(STILTS) tpipe \
               in='http://vizier.u-strasbg.fr/viz-bin/votable?-source=J%2fA%2bA%2f493%2f959&-oc.form=dec&-out.meta=DhuL&-out.max=1000000' \
               out=$@

BELLINI_CMD = $(STILTS) -allowunused plot2plane \
              in1=bellini.fits x1='Bmag-Vmag' y1='Vmag' \
              yflip=true \
              legend=false \
              size1=2 \
              compositor=0 \
              minor=false \
              out=$@ \
              layer.label=label color.label=black \
              fontsize.label=24 \
              x.label=x y.label=y \

CLOUD_CMD = $(BELLINI_CMD) icmd1='select Mm>=70' \
            xmin=-0.4 xmax=2.0 ymin=11 ymax=23 \
            in.label=cloud-point.csv ifmt.label=csv \
            auxvisible=false insets=0,0,1,1 xpix=400 ypix=400

WEIGHT_CMD = $(BELLINI_CMD) auxfunc=square auxmap=cold auxclip=0.1,1 \
             fontsize=20 texttype=antialias \
             ymin=11 ymax=23 xmin=-.9 xmax=3.5 \
             in.label=weight-point.csv ifmt.label=csv \

cloud-point.csv:
	echo x,y >$@
	echo -0.3,11.8 >>$@

weight-point.csv:
	echo x,y >$@
	echo -0.8,11.8 >>$@
 
cmd-flat.png: $(CMD_DATA)
	$(CLOUD_CMD) label.label='"Flat"' \
                     layer1=mark shading1=flat

cmd-tran.png: $(CMD_DATA)
	$(CLOUD_CMD) label.label='"Transparent"' \
                     layer1=mark shading1=transparent opaque1=20

cmd-cont.png: $(CMD_DATA)
	$(CLOUD_CMD) label.label='"Contour"' \
                     layer1=contour nlevel1=8 smooth1=20 scaling1=log \
                     color1=black

cmd-grid.png: $(CMD_DATA)
	$(CLOUD_CMD) label.label='"Grid"' \
                     layer1=grid xbinsize1=0.05 ybinsize1=0.2 combine1=count \
                     auxfunc=log auxmap=inferno auxclip=0.18,1

cmd-dens.png: $(CMD_DATA)
	$(CLOUD_CMD) label.label='"Density"' \
                     layer1=mark shading1=density \
                     densefunc1=log densemap1=inferno denseclip1=0.18,1

cmd-auto.png: $(CMD_DATA)
	$(CLOUD_CMD) label.label='"Auto"' \
                     layer1=mark shading1=auto


cmd-waux.png: $(CMD_DATA)
	$(WEIGHT_CMD) label.label='"Aux"' \
                      insets=7,0,9,1 xpix=401 ypix=410 auxvisible=false \
                      layer1=mark shading1=aux aux1=Mm

cmd-wgri.png: $(CMD_DATA)
	$(WEIGHT_CMD) label.label='"Grid"' \
                      insets=7,0,9,1 xpix=401 ypix=410 auxvisible=false \
                      layer1=grid weight1=Mm combine1=median \
                      xbinsize1=0.075 ybinsize1=0.2 

cmd-weig.png: $(CMD_DATA)
	$(WEIGHT_CMD) label.label='"Weighted"' \
                      insets=7,0,9,70 xpix=470 ypix=410 \
                      auxvisible=true auxlabel='' auxcrowd=0.8 \
                      layer1=mark shading1=weighted weight1=Mm combine1=median

fig-cloud.png: $(CLOUD_PANELS)
	montage $(CLOUD_PANELS) -tile 3x2 -geometry +0+0 $@

fig-weight.png: $(WEIGHT_PANELS)
	montage $(WEIGHT_PANELS) -tile 3x1 -geometry +0+0 $@




